Language Model Pre-Training with Sparse Latent Typing

Modern large-scale Pre-trained Language Models (PLMs) have achieved tremendous success on a wide range of downstream tasks. However, most of the LM pre-training objectives only focus on text reconstruction, but have not sought to learn latent-level interpretable representations of sentences. In this paper, we manage to push the language models to obtain a deeper understanding of sentences by proposing a new pre-training objective, Sparse Latent Typing, which enables the model to sparsely extract sentence-level keywords with diverse latent types. Experimental results show that our model is able to learn interpretable latent type categories in a self-supervised manner without using any external knowledge. Besides, the language model pre-trained with such an objective also significantly improves Information Extraction related downstream tasks in both supervised and few-shot settings. Our code is publicly available at: https://github.com/renll/SparseLT.

==> 1introduction.tex <==
\section{Introduction}

% \heng{TODOs: 1. change the design to bipartite graph: two layers, the first is entity-centric information network where each node is an entity and each edge is entity-entity relation; the second is event-centric information network where each node is an event and each edge is event-event relation. Event argument roles can be used to connect these two layers. Maybe the information passing and propagation can be done iteratively between these two layers 2. read Hanghang's paper. 3. Tasks to add: perhaps fine-grained entity typing; 4. need to futher expand the data size; 5. Story for introduction: to better profile an entity, we need to track their activities, because not all activities are reflected in traditional KG (entities and their relatively static relations; in the past event information was not used also because there is no large amount of event annotated data, but now we have relatiely mature event extraction system, so we construct a large-scale event annotated data automatically...}

% \heng{I found calling 'original KG' is a bit strange. need to re-word it throughout the paper. I don't have a good suggestion yet.}
% \textcolor{blue}{[HW: add one citation for each application]}
Knowledge graph (KG) is a kind of efficient and informative representation of structured knowledge.
A typical KG consists of a collection of knowledge triples, where each triple $(h, r, t)$ describes that the head entity $h$ and tail entity $t$ are connected through a relation $r$.
Recently, extensive studies have been focusing on knowledge graph representation learning, which aims to learn low-dimensional entity and relation embeddings that are informative and scalable to use for many downstream applications, such as information retrieval~\cite{irkg}, recommendation systems~\cite{recommenderkg}, machine reading comprehension~\cite{machinereadingkg}, and query-answering systems~\cite{qakg,qakg2}.
Typical KG embedding models, such as \cite{transe,conve,rotate}, usually learn the model parameters by maximizing pre-defined score functions on ground-truth triples.
One major limitation of such methods is that each knowledge triple is modeled locally and independently, without considering the global contextual information of KGs.
To solve this problem, another line of approaches~\cite{rgcn,compgcn} manages to model KGs as heterogeneous networks, and design message passing among entities using graph neural networks to better utilize global structural information.

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/example.pdf}
    \caption{An example of representing an event-enhanced KG as a heterogeneous network.}
    \vspace{-15pt}
    \label{fig:example}
\end{figure}
% \heng{maybe use different shapes to indicate entities and events so it's clear in the print out version}
However, the relations in knowledge graphs are mostly static factual connections between entities, which are still not sufficient for KG embedding models to learn fully rich and comprehensive entity representations.
% \han{This is not a full sentence per se. I was mainly confused by the "and" between static and factual connections. Maybe we can split it into two?}
If we think of how humans understand a real-world entity, we usually consider not only its static facts and properties, but more importantly, the dynamic \emph{events} associated with the entity as well.
Based on this motivation, we hypothesize that \emph{events} are essential for the model to understand entities and relations more comprehensively and improve the quality of KG embeddings, which can be beneficial for multiple knowledge-related downstream tasks.

In Information Extraction (IE), an \emph{event} usually consists of an \emph{event trigger} (a word or phrase that most directly indicates an event occurrence) and a set of \emph{event arguments} (the entities participating in the event with different roles), such as the \emph{Winning}, \emph{Awarded}, and \emph{Air Crash} events shown in Figure~\ref{fig:example}.
In general, events can benefit KG modeling mainly in the following four aspects: 
\begin{itemize}
    \item Events contain much richer information compared to the entity-entity relations in KG. For example, in Figure~\ref{fig:example}, the \emph{Awarded for films} event can give us a new aspect of the basketball player \emph{Kobe Bryant} for his excellence in films, while the relations in regular KGs only contain his well-known facts on sports.
    
    \item Compared with the triples in KGs which can only involve two entities, events are able to capture relations among multiple entities (depending on the number of arguments of this event) and thus they have more expressive power than traditional knowledge triples. For example, in Figure \ref{fig:example}, the event \emph{Winning Championship} connects three entities (\emph{NBA}, \emph{Lakers}, and \emph{Kobe Bryant}) together.
    
    \item Events can help improve the connectivity of KGs and mitigate the ubiquitous sparsity issue in most KGs. An event can reduce the distance between its two argument entities to 2 even if they are far away in original KGs. Events can also introduce more links to low-degreed or isolated entities (e.g., \emph{Oscar} and \emph{A helicopter} in Figure~\ref{fig:example}) to enrich KGs.
    
    \item In general, events that are related to each other can be organized in chronological order. The event-event temporal relations can also be incorporated to inform the model with the dynamic state transitions of entities. For example, in Figure~\ref{fig:example}, the original KG only contains the outdated information when \emph{Kobe Bryant} is still a basketball player. However, the event sequence $Winning \rightarrow Awarded \rightarrow Air Crash$ can provide information of \emph{Kobe}'s life at different stages, thus it will be greatly helpful for learning a more comprehensive entity representation.
\end{itemize}
% \han{Besides these three points, we can also mention that due to the introduced links, it benefits the message-passing as well. For example, for two nodes connected by a path of length 4, with the introduced event node it only takes 2 hops in the message-passing, hence reducing the depth requirement in GNNs, making the optimization easier.}
% \hh{if i understand correctly, what we really encode is event-adjacency info (e.g. which events happen around the similar time), right? Here is the dynamic kg embedding paper i mentioned \url{https://www.aaai.org/AAAI21Papers/AAAI-10116.YanY.pdf}. it is for a totally different applicatin (kg alignment). some components (mask/highway gates, fine-tuning) might be remotely related to this paper.  }
% \hh{an additional advantage might be in by introducing event node, we are able to capture high-order relation (as opposed to binary relationship in 'regular' kg), i.e., not including the event and related links?}
% In Information Extraction (IE) community, an event typically consists of an \emph{event trigger} (a word or phrase that most directly indicates the event occurrence) and its \emph{arguments} (entities participating in the event with different roles). 
% For example, in Figure~\ref{fig:example}, an \emph{Awarded for Oscar} event is occurred with three entity connected as arguments: \emph{Kobe Bryant}, \emph{Basketball}, and \emph{Los Angeles}, which indicates that \emph{Kobe Bryant is awarded Oscar in Los Angeles for his basketball-themed film.}
% We can discover that apart from static relations in the original KG, i.e., the gray nodes and edges that indicate some static properties for entities in Figure~\ref{fig:example}, events can help the model to understand entities in completely new perspectives.
% For example, such an \emph{Awarded for Oscar} event could provide us a brand new impression for the well-known basketball player \emph{Kobe Bryant} in the field of film and television art.
% If we manage to incorporate such events into KG embedding models, it would be greatly beneficial for a more comprehensive understanding of the existing entities and relations, and thus will lead to higher-quality KG representations.
% \heng{can your method deal with entities which are not linkable to KB? it will be important to clarify}

In this paper, we propose EventKE, an event-enhanced knowledge graph embedding model to incorporate event information into KG representations.
As shown in Figure~\ref{fig:example}, events are considered as an additional set of nodes beyond the original KG. Event nodes and entity nodes are distributed on two sides, and they are inter-connected by event argument links.
Moreover, event nodes and entity nodes are inner-connected by KG relations and event-event temporal links, respectively.
Inspired by graph attention networks~\cite{gat}, we design a four-stage attention-based information aggregation model to fuse event information into KG embeddings.
Specifically, we first calculate event embeddings based on entity embeddings using a left-to-right graph attention mechanism on event argument links, and then update event embeddings based on event-event temporal links. 
After that, the entity representations are updated by first passing back the event information and then conducting information aggregation through entity-entity relations. 
% \heng{unclear what you mean by 'aggregating back'}
The entire model is trained end-to-end by optimizing the convolutional-based distance function on ground-truth KG triples.

A practical challenge of applying event information to KG embedding is the scarcity of high-quality event annotations, since it is usually expensive to acquire manual event annotations that are relevant to KG entities.
Fortunately, as the event extraction techniques have become mature recently, we can manage to use event extraction systems to extract our desired events from natural language texts with high quality.
In this paper, in addition to the gold-standard event annotations such as those in the ACE-2005 dataset\fnurl{}{https://catalog.ldc.upenn.edu/LDC2006T06}, we also use a state-of-the-art cross-document event extraction and tracking system~\cite{resin} to obtain events from news articles.
This shows that our proposed EventKE can also be widely applicable to traditional KG datasets without manually-labeled events.
We evaluate our trained KG embeddings on three typical tasks: \emph{knowledge graph completion}, \emph{entity classification} and \emph{relation classification}, and the results demonstrate that the event information greatly improves knowledge graph representations.

% Since event annotations are usually expensive, in addition to the gold-standard events such as in the ACE-2005 dataset\fnurl{}{https://catalog.ldc.upenn.edu/LDC2006T06}, we also use the state-of-the-art event extraction system~\cite{resin} to extract events from texts.
% We adopt the typical relation-aware graph convolution networks~\cite{rgcn, compgcn} to model the static relations for KG representation learning.
% To make better use of event information, we consider events as additional \textbf{hyperedges}~\cite{hypergraphgnn} connecting multiple entity nodes.
% Each event is treated as an asymmetric hyperedge that connects all argumented entities with different roles.
% Based on such a type of event model, we design an attention-based hypergraph information aggregation method to model the message passing through hyperedges in graph neural networks.
% In specific, we first aggregate information from entities to event hyperedges through attention mechanisms, and then use the obtained hyperedge representations to aggregate back to update entity representations.

Our contributions can be summarized as follows:
\begin{itemize}
    \item We propose to incorporate event information into KG representation learning, and design a novel and effective attention-based bipartite information aggregation model to utilize the event information effectively.
    \item We demonstrate the effectiveness of EventKE by conducting experiments on multiple evaluation tasks. Experimental results show that incorporating events can significantly improve the learned KG embeddings compared with previous models. In specific, EventE achieves 13.4\% average relative gain on KG completion, 3.5\% absolute accuracy gain on entity classification, and 1.6\% absolute accuracy gain on relation classification, respectively.
    % \han{why using relative gain here but absolute gains later? Better to be consistent. Absolute values are more informative IMO.}
\end{itemize}












==> 2problem.tex <==
\begin{figure*}[tbp]
    \centering
    \includegraphics[width=0.99\textwidth]{figures/scheme.pdf}
    \caption{An illustration of the four-stage event-aware information aggregation model.}
    %\heng{label each box, indicate which one is amr graph, which one is external kb, etc.}}
    \vspace{-15pt}
    \label{fig:scheme}
\end{figure*}

\section{Problem Definition}
A knowledge graph is denoted by $G=(V,E)$, where $v_i\in V$ denotes the $i$-th entity node and $(i,j)\in E$ denotes the relation between the $i$-th entity node and the $j$-th entity node. 
We use $r_{i,j}\in\mathcal{R}$ to denote the relation type for edge $(i,j)$, such as the relation types \emph{team}, \emph{league}, and \emph{citizen} in Figure~\ref{fig:example}, where $\mathcal{R}$ represents the pre-defined relation type category.
Such a knowledge graph $G$ can also be represented by a collection of decomposed knowledge triples $\mathcal{G}=\{(v_i,r_{i,j},v_j)\}_{v_i,v_j\in V, r_{i,j}\in\mathcal{R}}$. 
% \hh{does your kg only contain entity and entity-entity relationship? }

To model the events, we treat events as an additional set of event nodes with event temporal relations.
We use $\mathcal{E}$ to denote the set of event nodes, where each event $e_j\in \mathcal{E}$ is composed of an event trigger $t_j$, its event type $c_j\in\mathcal{C}$, and a set of event arguments $A_j$.
The event trigger $t_j$ is a word or phrase from the original sentence that most clearly indicates the event occurrence, e.g., \emph{``wins''} for an event \emph{Winning Championship}, which is already included when the events are annotated or extracted from the original texts.
The event type $c_j$ is from a pre-defined event type category $\mathcal{C}$, such as the \emph{Winning Championship} and \emph{Awarded for films} for the first two event nodes in Figure~\ref{fig:example} respectively.
The set of event arguments $A_j$ is composed of a set of pairs of entities and event argument roles.
\begin{equation*}
    A_j=\left\{\left(v_{j,k},z_{j,k}\right)\right\}_{k=1}^{|A_j|},
\end{equation*}
where $|A_j|$ is the number of arguments for event $e_j$. 
$v_{j,k}\in V$ denotes the entity of the $k$-th argument for event $e_j$, and $z_{j,k}\in \mathcal{A}$ denotes the role type (also from a pre-defined collection of role types $\mathcal{A}$) for this entity in event $e_j$.
For example, (\emph{``Kobe Bryant''}, \emph{winner}) and (\emph{``Oscar''}, \emph{award}) in Figure~\ref{fig:example} are two event arguments for the event \emph{Awarded}.

The objective of event-enhanced KG embedding is to learn a low-dimensional representation vector $\bm v_i$ for each node $v_i\in V$ with the help of the original knowledge graph $G$ and the events $\mathcal{E}$.


==> 3method.tex <==
% \section{Approach}

% two-column figure template
% \begin{figure*}[tbp]
%  \centering
%  \includegraphics[width=1\textwidth]{figures/scheme.pdf}
%  \caption{Overview of our proposed framework for biomedical information extraction.}
%  \vspace{-15pt}
%  \label{fig:scheme}
% \end{figure*}
\section{Model}
% \subsection{Embedding Initialization}
% We initialize the embeddings for each entity $v_i\in V$ and each event trigger $t_k$ using pretrained BERT~\cite{bert} and denote them as $\bm v_i^0$ and $\bm t_k$ respectively.
% For entities and event triggers with multiple mentions, we average the BERT embeddings of all mentions as the final representation vector.
% Also, we randomly initialize the representation vectors for relation types $\mathcal{R}$, event types $\mathcal{T}$, and argument types $\mathcal{A}$ and obtain the embeddings $\bm r_{i,j}$, $\bm c_k$, and $\bm \alpha_{k,p}$, which are optimized in training. 
\subsection{Overview}
Given a knowledge graph $G=(V,E)$ and a set of events $\mathcal{E}$, we consider events as an additional set of nodes, and build a heterogeneous network where the entity nodes $V$ and event nodes $\mathcal{E}$ are distributed on two sides.
As shown in Figure~\ref{fig:scheme}, the entity nodes and event nodes are inter-connected by event argument links, while both of the entity set and event set are also inner-connected by relations from the original KG and event-event temporal links, respectively.
We design an $L$-layer event-aware bipartite information aggregation model to enforce the entities to aggregate information from both knowledge graph neighbors and relevant events, where the illustration for each layer is shown in Figure~\ref{fig:scheme}.
The whole model is trained end-to-end by optimizing the convolution based scoring function on ground-truth knowledge triples with output embeddings from the last layer.

\subsection{Event-aware Information Aggregation}
As shown in Figure~\ref{fig:scheme}, given the heterogeneous network with entity and event nodes, each layer of the event-aware bipartite information aggregation model consists of four stages.
First, we compute the event representations using a graph attention mechanism on the event argument links.
Then, we conduct message passing on the event nodes with temporal relations to update the event representations.
After that, we aggregate the event information back to the entities based on another graph attention mechanism on event argument links.
Finally, the entity representations are updated by incorporating the event information and the neighborhood message from the original KG relations. 
% \hh{this 'co-attention' mechanism is interesting. reviewers might wonder -- why not run GAT on the entire heterogeneous network? in this way, we can also let different event/entity node to attend each other, with a more succinct model (as opposed to two GAT + two GCNs). do we have any explanation and/or empirical evidence to support the proposed design?}

We use $\bm v_{i}^{l}$ to denote the representation vector for the $i$-th entity in layer $l$, and the relation type embedding is denoted as $\bm r_{i,j}$.
We use $\bm t_j$, $\bm c_j$ to denote the embedding vectors for the event trigger and event type of event $e_j$ respectively.
For event arguments, since each of them is also an entity, we use $\bm v_{j,k}^{l}$ to represent the embedding for the $k$-th argument of event $e_j$, and the corresponding role type embedding is denoted as $\bm z_{j,k}$.
Note that only the entity embeddings are updated in each layer, while other embeddings are identical in each layer and uniformly optimized through end-to-end training to reduce the model size. 
% \hh{do we need any justification for this, e.g., why fixing event embedding across layers?}

\paragraph{Information aggregation from entities to events.}
We first use an entity-to-event graph attention mechanism to aggregate entity information to events through the event argument links.
For each event $e_j$ with the number of arguments $|A_j|$, we first compute the attention weights $\alpha_{j,k}$ according to the concatenation of embeddings of event trigger, event type, entity, and role type:
\begin{equation}
    \alpha_{j,k}=\frac{\exp \sigma\left(\textbf W_{\alpha}\left[\bm t_j, \bm c_j, \bm v_{j,k}^{l}, \bm z_{j,k}\right]\right)}{\sum\limits_{p=1}^{|A_j|}\exp\sigma\left(\textbf W_{\alpha}\left[\bm t_j, \bm c_j, \bm v_{j,p}^{l}, \bm z_{j,p}\right]\right)},
\end{equation}
% \han{Is there any specific consideration to use leaky ReLU here?}
where $\sigma(\cdot)$ is a \emph{LeakyReLU} activation function as in~\cite{gat}, and $\textbf{W}_{\alpha}$ denotes a trainable parameter for linear transformation.
Here, $\bm v_{j,k}^{l}$ denotes the entity embedding for the $k$-th event argument for event $j$.
Such an attention mechanism is capable of incorporating rich event information including event trigger, event type, and argument role types.
Then the entity information $\bm{\lambda}_j$ passing to each event $e_j$ from its arguments can be computed by the following weighted sum:
\begin{equation}
    \bm \lambda_j=\sum_{k=1}^{|A_j|}\alpha_{j,k}\sigma_e\left(\textbf W_e\bm v^{l}_{j,k}\right),
\end{equation}
where $\sigma_e(\cdot)$ denotes the \emph{ReLU} activation function and $\textbf{W}_e$ is a trainable matrix.
We concatenate the event trigger embedding $\bm t_j$, event type embeddings $\bm c_j$ , along with the entity information vector $\bm \lambda_j$, as the event representation $\bm e_j$:
\begin{equation}\label{eqn:eventrepr}
    \bm e_j=\left[\bm t_j, \bm c_j, \bm \lambda_j\right].
\end{equation}

\paragraph{Message passing on event-event relations.}
We then update the event representations $\bm e_j$ by conducting message passing on event-event temporal links.
We use $\mathcal{N}(j)$ to denote the set of event nodes that have temporal relations with $e_j$, then the event representation is updated similar to graph convolution network~\cite{gcn}.
\begin{equation}\label{eqn:event-event}
    \widetilde{\bm e}_j=\bm e_j + \gamma\cdot\sigma_e\left(\frac{1}{|\mathcal{N}(j)|}\sum_{k\in \mathcal{N}(j)}\bm e_k\textbf W_t\right),
\end{equation}
where $\gamma$ is a hyper parameter controlling the amount of information to incorporate from event neighbors.
Such a message passing procedure can efficiently inform the model with event-event temporal information.

\paragraph{Information aggregation from events to entities.}
After we obtain the event representations $\widetilde{\bm e}_j$, we use another graph attention mechanism to aggregate event information back to entities.
For each entity $v_i$, we use $\mathcal{E}_i$ to denote the set of events that are connected with $v_i$ through event arguments:
\begin{equation}
    \mathcal{E}_i=\left\{e_j  \mid \exists ~1\leqslant k \leqslant |A_j|, v_i=v_{j,k}\right\}.
\end{equation}
For example, in Figure~\ref{fig:scheme}(c), the $\mathcal{E}_i$ for node $v_i$ should be $\{e_{j}, e_{j+1}, e_{j+2}\}$.
We manage to fuse the event information back to involved entities using an attention mechanism, where the attention weight $\beta_{i,k}$ for event $e_k$ is computed by
\begin{equation}
    \beta_{i,k} = \frac{\exp \sigma\left(\textbf W_{\beta}\left[\widetilde{\bm e}_k, \bm v_{i}^{l}\right]\right)}{\sum\limits_{p=1}^{|\mathcal{E}_i|}\exp \sigma\left(\textbf W_{\beta}\left[\widetilde{\bm e}_p, \bm v_{i}^{l}\right]\right)},
\end{equation}
where $\sigma(\cdot)$ and $\textbf{W}_{\beta}$ denote the \emph{LeakyReLU} activation function and the linear transformation parameter respectively.
Then we compute the event information $\widetilde{\bm v}_i$ for entity node $v_i$ by weighted sum:
\begin{equation}
    \widetilde{\bm v}_{i} = \bm v_{i}^{l}+\epsilon\cdot\sum_{k=1}^{|\mathcal{E}_i|}\beta_{i,k}\textbf W_v \widetilde{\bm e}_k.
\end{equation}
Similar to Eq.~\eqref{eqn:event-event}, we also adopt a hyper parameter $\epsilon$ to control the message passing level from events to entities.
The event information vector $\widetilde{\bm v}_i$ is supposed to contain rich information from events, including event triggers, event types, argument roles and also the event temporal relations.

\paragraph{Message passing on entity-entity relations.}
In the final stage, we conduct message passing on the original entity-entity relations from the original KG to further incorporate information from the original static relations between entities.
To handle the different relation types, we adopt Composition GCN~\cite{compgcn} to model the relation types using different relation type embeddings.
We use $\mathcal{N}(i)$ to denote the set of entity nodes that are connected with $v_i$ through the original entity-entity relations in knowledge graphs, and the entity representations are updated by
\begin{equation}
    \bm v^{l+1}_{i}=\sigma_e\left(\sum_{j\in\mathcal{N}(i)\cup\{i\}}\textbf W_r \phi\left(\widetilde{\bm v}_{j},\bm r_{i,j}\right)\right),
\end{equation}
where $\sigma_e(\cdot)$ is the \emph{ReLU} activation function, $\bm r_{i,j}$ is the relation type embedding, and $\phi(\cdot)$ denotes a circular correlation operator\footnote{The circular correlation $\phi(a,b)$ between two vectors $a$ and $b$ is defined as $[\phi(a,b)]_k=\sum_{i=0}^{d-1}a_i b_{(k+1)~mod~d}$, where $d$ denotes the dimension of the vectors. }~\cite{circulargcn} between two vectors.
Finally, we obtain the updated entity representation $\bm v_{i}^{l+1}$ that incorporates both the information from the original KGs and the rich event information from event nodes.
We use the final layer output $\bm v^{L}_{i}$ for model optimization and knowledge graph representation learning.

\subsection{Optimization}
After we obtain the entity representations $\bm v_{i}^{L}$ and relation type embeddings $\bm r_{i,j}$, the model is optimized by maximizing the convolution-based score function for each knowledge triple $( v_{i},  r_{i,j}, v_{j})$.
Basically given each head entity $v_i$ and the relation $r_{i,j}$, we use $\mathcal{V}^+$ to denote the set of all possible tail entities, and use $\mathcal{V}^-$ to denote the set of random sampled negative entities.
Then the loss for such a triple can be computed by binary cross-entropy: 
\begin{equation*}
\begin{split}
    & \mathcal{L}\left(v_{i}^{L}, r_{i,j}\right)\!=\!-\!\!\sum_{v_+\in \mathcal{V}^+}\!\log\sigma_s \left(\textsc{conv}\!\left(\bm v_{i}^{L}, \bm r_{i,j}, \bm v_{+}^{L}\right)\right)  \\ 
    & - \sum_{v_-\in \mathcal{V}^-}\log\left(1-\sigma_s\left(\textsc{conv}\!\left(\bm v_{i}^{L}, \bm r_{i,j}, \bm v_{-}^{L}\right)\right)\right) \\
\end{split}
\end{equation*}
where $\sigma_s$ is the sigmoid function, and $\textsc{conv}(\cdot)$ is the convolution based scoring function defined in~\cite{conve}.
Specifically, given a knowledge triple $(\bm s,\bm r,\bm t)$, the score function can be computed by $\textsc{conv}(\bm s, \bm r, \bm t)=f\left(\textup{vec}\left(f(\left[\overline{\bm s},\overline{\bm r}\right]*\omega)\right)\textbf W\right)\bm t$, where $\overline{\bm s}$ and $\overline{\bm r}$ denote the 2D reshaping for vectors and $*$ denotes the convolution operator.
% \han{I assume the $*$ means the convolution operator, but we haven't properly introduced this notation so far.}








==> 4experiment.tex <==
% \section{Experiments}
\section{Experiments}


\heng{give qualitative analysis with examples instead of just numbers and visualization}

\subsection{Dataset}
We first evaluate our model on the Automatic Content Extraction (ACE 2005) dataset,\fnurl{}{https://catalog.ldc.upenn.edu/LDC2006T06} which provides document-level entity, relation, and event annotations.
We use this dataset because it has gold-standard event annotations, which is convenient to evaluate the impact of incorporating events into KG embeddings.
We perform automatic entity linking~\cite{blink} to link the entities to Wikidata (dumped in August 2019), and merge the entities with the same Wikidata entries into one single node.
We use the most recent event-event temporal relation extraction system~\cite{temporal2021} to obtain the event-event temporal relations. 
% \heng{which Wikipedia dump? put in date}

However, gold-standard event annotations for real-world KGs are usually expensive or even intractable.
To demonstrate that our proposed model can also be applied to KGs without gold-standard event annotations, we choose another large-scale dataset, WikiEvents~\cite{docie2021}, which contains %event-centric Wikipedia 
news articles from Wikipedia references about complex events.
We use the most recent cross-document event extraction~\cite{oneie,docie2021}, coreference resolution~\cite{Tuan2021} and temporal tracking system~\cite{resin} to automatically extract events from the news articles.

The statistics of the extracted KGs from the two datasets are shown in Table~\ref{tab:dataset}.

\begin{table}[htbp]
	\centering
    \small
	\begin{tabular}{c|cccc}
		\toprule[1pt] 
		Dataset & Entities &  Rels &  Events &  Args \\
		\midrule[1pt]
		ACE-2005 & 7,376 & 7,441 & 3,071 & 5,587  \\
		\specialrule{0em}{1pt}{1pt}
		\hline
		\specialrule{0em}{1pt}{1pt}
        WikiEvents & 104,942 & 151,253 & 39,092 & 112,972    \\

		\midrule[1pt]
	\end{tabular}
	\normalsize
	\caption{The statistics of the extracted knowledge graphs from the two datasets, where \emph{Rels} and \emph{Args} denote the number of entity-entity relations and event argument links respectively.}
	\label{tab:dataset}
\end{table}


\subsection{Evaluation Tasks}
We evaluate our trained knowledge graph embeddings on three typical evaluation tasks: \emph{knowledge graph completion}, \emph{entity classification}, and \emph{relation classification}.
\paragraph{Knowledge Graph Completion}
KG completion~\cite{transe} is a typical task for evaluating knowledge graph embeddings, which aims to predict the tail entity $t$ given a pair of head entity $h$ and relation $r$. 
Since the number of entities in KG is usually large, we use the ranking based metrics~\cite{transe}: mean ranking (MR), mean reciprocal ranking (MRR), and Hits@k to evaluate the KG completion performance.
For WikiEvents dataset with extremely large number of entities, it is not scalable to evaluate among all entities, therefore, we randomly selected a fixed number of negative samples and calculate the rankings of the correct tail entity.
\paragraph{Entity Classificiation}
The entity classification task aims to classify each entity node into a pre-defined entity type category.
We divide all entities in the KG into 80\% training, 10\% validation, and 10\% testing examples.
After we obtain our trained KG embedding, we adopt a two-layer feed-forward neural network with \emph{ReLU} activation on the hidden layer on the top of our model to fine-tune for entity classification task on the training entities, and select the best model on the validation set, then report the entity classification accuracy on the testing entities. 
There are totally 45 fine-grained entity types in \emph{ACE-2005} dataset and 9 types in \emph{WikiEvents}.
% In ACE 2005 dataset, each entity is classified into the pre-defined 7 entity types:
% We only consider entity mentions with their pre-defined entity type categories.
% \heng{list entity type categories} \heng{are you classifying entity mentions or entity clusters? did you include name, nominal and pronoun mentions?}
\paragraph{Relation Classification}
The relation classification task aims to identify the relation type between each given pair of entities.
Similar to entity classification, we also divide all the entity-entity relations into training, validation, and testing sets and use a two-layer feed-forward neural network for relation classification, and use the accuracy as the evaluation metric.
There are totally 18 relation types in \emph{ACE-2005} dataset and 9 types in \emph{WikiEvents}.


\subsection{Baselines and Implementation Details}
\paragraph{Baselines}
We first adopt the most typical previous models \textbf{\emph{TransE}}~\cite{transe} and \textbf{\emph{CompGCN}}~\cite{compgcn} as the representatives of translation based and graph neural network based KG embedding models respectively.
In both of these two methods, we only use the initial KG and the entity-entity relations without any events, and the entity node embeddings are randomly initialized before training.
To show the influence of incorporating the pretrained language model BERT~\cite{bert}, in \textbf{\emph{CompGCN-BERT}}, we use the \emph{bert-base-uncased} model checkpoint\fnurl{}{https://huggingface.co/bert-base-uncased} to initialize entity node embeddings before conducting message passing using CompGCN.
For our event-enhanced models, \textbf{\emph{EventKE}} represents our proposed event-enhanced knowledge graph embedding model.
In addition, to show the effects of each individual part of our model, we also introduce two model variants for ablation study.
\textbf{\emph{EventKE-w/o-templink}} denotes the model without information aggregation on event-event temporal links. 
In \textbf{\emph{EventKE-w/o-events}}, instead of using annotated events or event extraction results, we randomly initialize all events (including the event triggers, event types, and event arguments) and the use such ``random events'' to train the model.
Note that the number of model parameters in \textbf{\emph{EventKE-w/o-events}} and \textbf{\emph{EventKE}} are exactly the same, we want to evaluate whether the performance gains come from the valuable event information, or merely come from the larger capacity of the whole model.

\paragraph{Implementation Details}
We train the KG embedding models for a maximum of $200$ epochs and apply an early stopping strategy of $10$ epochs (if the validation loss is not lower than the previous best for $10$ consecutive epochs, we will stop training the model).
We train the models on NVIDIA Tesla V100 GPUs using the Adam~\cite{adam} optimizer with a learning rate of $10^{-4}$.
The average runtime is about 3 hours for the \emph{ACE-2005} dataset and 5 days for the large KG in the \emph{WikiEvents} dataset.
The detailed hyper-parameter choices are shown in Appendix A.

\subsection{Results}


\begin{table*}[h]
	\centering
	\vspace{5pt}
	\small
	\begin{tabular}{c|c|c|c|c|c|c|c|c}
% 	\small
		\toprule[1.5pt] 
		Dataset & \multicolumn{4}{|c|}{\textbf{\emph{ACE-2005}}} & \multicolumn{4}{|c}{\textbf{\emph{WikiEvents}}} \\
		\specialrule{0em}{1pt}{1pt}
		\cline{1-9}
		\specialrule{0em}{1pt}{1pt}
		Metrics  & MRR &  MR  & Hits@10 & Hits@20
		& MRR &  MR  & Hits@10 & Hits@20\\
		\midrule[1pt] 
		TransE~\cite{transe} & 0.095 & 112  & 0.181 & 0.223 & 0.067 & 213  & 0.111 & 0.153\\
		\specialrule{0em}{1pt}{1pt}
		\hline
		\specialrule{0em}{1pt}{1pt}
		CompGCN~\cite{compgcn} & 0.102 & 88.8  & 0.201 & 0.256 & 0.074 & 186  & 0.134 & 0.171\\
		CompGCN-BERT & 0.178 & 79.5  & 0.322 & 0.419 & 0.149 & 168  & 0.210 & 0.259  \\
		\specialrule{0em}{1pt}{1pt}
		\hline
		\specialrule{0em}{1pt}{1pt}		
		\textbf{EventKE} (Ours) & \textbf{0.203} & \textbf{67.5}  & \textbf{0.378} & \textbf{0.480} & \textbf{0.168} & \textbf{147}  & \textbf{0.257} & \textbf{0.322} \\
		- w/o temporal links & 0.196 & 78.5  & 0.362 & 0.465 & 0.166 & 149  & 0.249 & 0.312  \\
		- w/o events & 0.181 & 78.9 & 0.111  & 0.408 & 0.146 & 168  & 0.210 & 0.242 \\

		
		\midrule[1pt]
		
% 	\normalsize

	\end{tabular}
		\caption{Knowledge graph completion performance. We set the number of negative samples as $K=500$.}
	\label{tab:kg_completion}
	\normalsize
	\vspace{-0.45cm}
\end{table*}

\begin{table}[tbp]
	\centering
% 	\vspace{-10pt}
    \small
	\begin{tabular}{c|cc|cc}
		\toprule[1pt] 
		Dataset & \multicolumn{2}{|c|}{\textbf{\emph{ACE-2005}}} & \multicolumn{2}{|c}{\textbf{\emph{WikiEvents}}} \\
		\specialrule{0em}{1pt}{1pt}
		\hline
		\specialrule{0em}{1pt}{1pt}
		 Model & Ents &  Rels  & Ents & Rels\\
		\midrule[1pt]
		 TransE & 70.25 & 56.32 &79.63  & 72.29\\
		CompGCN & 71.02 & 55.99 & 80.04 & 73.06\\
		\specialrule{0em}{1pt}{1pt}
		\hline
		\specialrule{0em}{1pt}{1pt}
		BERT-Only & 71.13 & 58.64 & 82.11  & 76.01\\
		CompGCN-BERT & 73.92 & 60.81 & 82.56 & 76.58\\
		\specialrule{0em}{1pt}{1pt}
		\hline
		\specialrule{0em}{1pt}{1pt}
		\textbf{EventKE} (Ours) & \textbf{77.47} & \textbf{62.60} & \textbf{85.61} & 77.94 \\
		
		- w/o temporal links & 75.81 & 62.20 & 84.32  & \textbf{78.11}\\
		- w/o events & 73.32 & 61.06 & 82.20 & 76.29 \\
		\midrule[1pt]
	\end{tabular}
	\normalsize
	\caption{Accuracy (\%) of entity and relation typing.}
	\vspace{-16pt}
	\label{table:entity_relation}
\end{table}

Table~\ref{tab:kg_completion} and Table~\ref{table:entity_relation} show the performance on knowledge graph completion, entity classification, and relation classification, respectively.
In general, our model significantly outperforms all baseline competitors.
By incorporating event information (compared with \emph{CompGCN-BERT}), our model can achieve 13.4\% average relative gain on KG completion MRR, and 3.5\% and 1.6\% absolute gain on entity and relation classification accuracy.

\paragraph{Effects of incorporating events.}
The evaluation results demonstrate that incorporating event information can greatly improve the quality of entity and relation embeddings.
From the results shown in Table~\ref{tab:kg_completion} and Table~\ref{table:entity_relation}, we can also find that event-event temporal links can also show effectiveness especially on the task of KG completion and entity classification.
We can also see that the performance of \emph{EventKE-w/o-event} is evidently lower than \emph{EventKE} on all tasks, even if it has the same number of model parameters with \emph{EventKE}.
Such results demonstrate that the performance gains come from the event information instead of larger model capacity.

\paragraph{Effects of using BERT.}
From the results, we can also find that \emph{CompGCN-BERT} performs much better that \emph{CompGCN}, which demonstrates that initializing the entity and event node embeddings using pertrained language models can significantly improve the performance.
This is probably because the BERT embeddings contain sentence-level contextual information of entity mentions and event triggers, which are not captured in pretraining in the random initialization setting.

\subsection{Qualitative Analysis}

\begin{table*}[t]
	\centering
	\vspace{5pt}
	\small
	\centering
	\begin{tabular}{m{6cm}|c|c|c}
% 	\small
		\toprule[1.5pt] 
		Sentence with events & Event Structure & Task Input & Ranking Change\\
		\specialrule{0em}{1pt}{1pt}
		\hline
		\specialrule{0em}{1pt}{1pt}
		Well, when they do finally enter {\color{brown}{Baghdad}}, U.S. and coalition troops could face urban {\color{blue}{combat}} with the {\color{brown}{Republican Guard}}, some of whom may have withdrawn into the city.  &\begin{minipage}{0.16\textwidth}

      \includegraphics[width=24mm, height=18mm]{figures/event_eg1.pdf}

    \end{minipage} & \begin{minipage}{0.15\textwidth}

      \includegraphics[width=26mm, height=20mm]{figures/input1.pdf}

    \end{minipage} & \begin{minipage}{0.15\textwidth}

      \includegraphics[width=26mm, height=20mm]{figures/rank1.pdf}

    \end{minipage} \\
        \specialrule{0em}{1pt}{1pt}
		\hline
		\specialrule{0em}{1pt}{1pt}
		{\color{brown}{Israel}} {\color{blue}{retaliated}} on {\color{brown}{Hamas}}, namely {\color{brown}{Al-Rantissi}}, it missed him and killed civilians.  &\begin{minipage}{0.15\textwidth}

      \includegraphics[width=26mm, height=22mm]{figures/event_eg2.pdf}

    \end{minipage} & \begin{minipage}{0.16\textwidth}

      \includegraphics[width=28mm, height=20mm]{figures/input2.pdf}

    \end{minipage} & \begin{minipage}{0.15\textwidth}

      \includegraphics[width=26mm, height=18mm]{figures/rank2.pdf}

    \end{minipage} \\
    
		
% 	\normalsize
		\midrule[1pt]
	\end{tabular}
		\caption{Qualitative examples from the validation set demonstrating how events can help on KG completion.}
	\label{tab:qualitative}
	\normalsize
	\vspace{-0.45cm}
\end{table*}
To further inspect how events help better understand the knowledge graph, we analyze the output results from the validation set of KG completion task, and show two typical examples in Table~\ref{tab:qualitative}.
Given an input head entity and a relation, we show the rankings of the correct tail entity before and after incorporating event information in the last column of Table~\ref{tab:qualitative}.

In the first example, the model is required to predict where the \emph{Republican Guard} is \emph{located in}, however, the entity-entity relations (in the training set) from the knowledge graph do not contain such information, which makes the model output a low ranking for the correct entity \emph{Baghdad}.
After incorporating event information, the entities \emph{Republican Guard} and \emph{Baghdad} are connected through a \emph{Conflict:Attack} event node, which indicates that \emph{Republican Guard} is currently located in \emph{Baghdad} to participate this attacking event.
As a result, the number of hops between these two entities is greatly reduced, and the model can successfully predict the correct tail entity based on such event information.

Similarly, in the second example, the model is asked to predict the \emph{membership} of \emph{Al-Rantissi}.
We can see that there is also a \emph{Conflict:Attack} event indicating that \emph{Isarel} targets to retaliate on \emph{Hamas} and \emph{Al-Rantissi}.
Although such an attack event can not directly indicate that \emph{Al-Rantissi} is a member of \emph{Hamas}, it can inform the model that \emph{Al-Rantissi} and \emph{Hamas} are strongly related since they have both been targeted in one single attack event.
Therefore, the ranking of \emph{Hamas} is greatly increased from $117$ to $3$, which contributes to the overall performance gain of KG completion.
% In summary, the events can help to improve the performance of KG completion by providing direct information or giving some implicit hints for the model to identify the correct target entity.







==> 5related.tex <==
\section{Related Work}
\paragraph{Knowledge Graph Embedding}
% Knowledge graph embedding (KGE) models aim to learn low-dimensional representation vectors for entities and relations in a knowledge graph.
The most traditional translation-based KG embedding models are first proposed by~\cite{transe}, which manage to model each knowledge triple as translation and train the model by minimizing the distance function between head entity, relation, and tail entity.
Previous translation-based models are mainly diverse in how to model the distance for each triple.
Typical methods include using relation hyperplanes~\cite{transh,transr}, projection matrix decomposition~\cite{transd,transsparse}, relational mappings~\cite{transm}, multiple relation projections~\cite{transf}, Gaussian distributions~\cite{gaussian,transg}, neural networks~\cite{distmult,complex}, 2D convolutions~\cite{conve,adapconv}, and rotations~\cite{rotate}. 
However, such translation-based methods model each knowledge triple individually without considering the global context for entities in the KG.
To solve this problem, another line of work attempts to model the KG as a unified heterogeneous graph and use graph neural networks to capture the global interactions between entity nodes, such as~\cite{circulargcn,rgcn,htgnn,compgcn,hgt,molecular}.
Recent studies also focus on using additional information to improve KG embedding, such as entity type information~\cite{autoeter} and text information~\cite{kepler}.
% \heng{add comparison and discussion}


\paragraph{Event Extraction and Utilization}
Events can help the KG embedding model to get a more comprehensive understanding of entities.
A variety of event extraction models are proposed to extract events from natural language texts, such as~\cite{liberalie,zero-shot,dygie,dygie++,oneie,docie2021}.
The dynamic event information is also well utilized in various areas, such as pretrained language models~\cite{eventplm}, event temporal information prediction~\cite{duration,temporal2021}, event schema induction~\cite{li-etal-2020-connecting}, and event network representation learning~\cite{eventnetwork}.
To the best of our knowledge, we are the first to focus on improving the entity and relation embeddings using event information in KG representation learning.

\paragraph{Comparison and Discussion}
Our approach is highly related to the global event network embedding model~\cite{eventnetwork}, however, there are a few essential differences.
First, \cite{eventnetwork} focuses on learning the embedding vectors for events to use for event-centric downstream tasks such as event type classification, argument extraction, and event coreference resolution.
Our model focus on using event information to improve entity and relation understanding in knowledge graphs.
For model design, \cite{eventnetwork} treats the entity and event nodes as a unified network, and adopts a relational GCN module to encode the entire network.
On the contrary, we regard the entities and events as two separate sets of nodes and conduct pairwise message passing between the two node sets.
In addition, compared to \cite{eventnetwork}, we manage to make use of a wider range of event information including the event types and event temporal relations.

==> 6conclusion.tex <==
\section{Conclusion and Future Work}
Relations in traditional KGs usually reflect only static and factual connections, which fail to incorporate dynamic activities and state changes about entities.
In this paper, we focus on incorporating \emph{events} into KG representation learning, and building a heterogeneous network by introducing an additional event node layer.
We design a novel and effective attention-based message passing method on entity-entity, event-entity, and event-event relations, to fuse the event information into KG embeddings. Experimental results on multiple evaluation tasks show the compelling effectiveness of incorporating events in KGs.
For future work, we will consider applying EventKE to more challenging event-related tasks, such as event schema induction.
In addition, using pretrained language models to jointly learn KG and text embeddings is also a promising direction.

==> backup/1.1taskimportance.tex <==



The task of Biomedical Information Extraction~\cite{poon-vanderwende-2010-joint,mcclosky-etal-2011-event-extraction,kim-etal-2013-genia,rao-etal-2017-biomedical,kb-driven-tree-lstm,espinosa-etal-2019-search,wang-etal-2020-biomedical,ramponi-etal-2020-biomedical,huang-etal-2020-biomedical} aims to extract entities and the relations and events involving them from scientific literature. It is a key task to create a dynamic knowledge base  to accelerate biomedical scientific discovery such as discovering new molecules. For example, practical progresses at combating COVID-19 highly depend on effective transmission, assessment and extension of these research results. 




%cite some of the recent papers at bionlp








==> backup/1.2challengessolutions.tex <==


Compared to general domains such as news, IE from scientific papers presents two unique and non-trivial challenges.
First, the authors of scientific papers tend to compose long sentences, where the event trigger and entity mentions are usually located far away within the sentence.
As shown in Table~\ref{tab:example}, we can see that compared with ACE05 dataset in news domain, the average distance between triggers and entities is much longer in biomedical scientific papers.
Therefore, it is more difficult for IE models to capture the global context only with the existing flat sequential sentence encoders.

Second, comprehending sentences from scientific papers highly requires external knowledge, because there are many domain-specific common expressions, acronyms and abbreviations that are difficult for the model to understand.
For instance, as shown in Figure~\ref{fig:example}, it is nearly impossible for a typical end-to-end model, which only takes in the sentence as input, to get clear understanding of \emph{CTF}, \emph{OTF-1}, and \emph{OTF-2} without background knowledge.
\begin{table}[htbp]
	\centering
    \small
	\begin{tabular}{ccc}
		\toprule[1pt] 
		Dataset & Average distance & Maximal distance  \\
		\midrule[1pt]
		ACE05-E & 0.211 sentence & 56 words  \\
		\specialrule{0em}{1pt}{1pt}
		\hline
		\specialrule{0em}{1pt}{1pt}
		GENIA-2011 & 0.349 sentence & 74 words \\
		\midrule[1pt]
	\end{tabular}
	\normalsize
	\caption{Comparison of the average distance (normalized by sentence length) and the maximum distance (measured by the number of tokens) between each trigger-entity pair in news domain (ACE-05 dataset) and scientific paper domain (GENIA-2011 dataset). \heng{for ACE data did you count the distance between trigger and entity mention for the same event mention? the number does not look right.}}
	\label{tab:example}
\end{table}










%example to show lack of external knowledge


%third challenge: domain-specific, fine-grained...


%%%%%%%%%%%%%%%COMMENTS%%%%%%%%%%%%%%%


% However, there are several challenges we found from the error analysis on the result of these experiments (Figure \ref{fig:error-oneie}). First, in this biomedical scientific domain, the entity is often represented by an acronym with a short length of characters (e.g., the entity proteins Baf-2 and RNA). This word representation makes the model easily overfitted when detecting these entities due to the word features' lack of variations. Second, the sentence structure and style on the scientific paper are domain specialized compared to the general domain, such as newspapers. As the content is more targeted to the knowledgeable reader, the language model style can differ for different scientific domains besides its author writing style. Finally, we found some error cases where the model failed to detect multiple entities sequentially in a sentence, especially if it doesn't have proper conjunction. This broken sentence structure becomes a challenge, which tells us that the BERT language model may not be enough for handling this case.

==> backup/1.3solution.tex <==
% Paragraph #3: How we address these two challenges (AMR and KG respectively), explain using the example.
To tackle these two challenges, we propose a novel framework for biomedical IE that integrates Abstract Meaning Representation (AMR)~\cite{banarescu13} \heng{add citation for AMR} and external knowledge graph. 
%\heng{need to explain what is AMR.} 
AMR is a semantic representation language, to convert the meaning of each input sentence into a rooted, directed, labeled, acyclic graph structure. AMR semantics includes PropBank frames, non-core semantic roles, coreference, entity typing and linking, modality, and negation. Compared with dependency parsing and semantic role labeling, the nodes in AMR are concepts instead of words, and the edge types are much more fine-grained. A large, labeled AMR corpus \heng{add LDC catalog} has been developed  for both general domain and biomedical scientific literature domain. We train an automatic AMR semantic parser using the algorithm XXX~\cite{} \heng{add citation}. To better handle long sentences with distant trigger and entity pairs, we use AMR parsing to compress the sentence and to better capture global interactions between tokens.
For example, as shown in Figure~\ref{fig:example}, the \emph{Positive Regulation} event trigger \emph{``changes''} is located far away from its arguments \emph{CTF}, \emph{OTF-1}, \emph{OTF-2} in the original sentence.
However, in the AMR graph, such trigger-entity pairs are linked within two hops.
Therefore, it will be much easier for the model to identify this kind of events with the guidance of AMR parsing.
In addition, to exploit the external knowledge, we extract a global knowledge graph from Comparative Toxicogenomics Database (CTDB) that covers all entity nodes in the corpus.
For each sentence, we select a minimal connected subgraph as the sentence-level KG and fuse it with the AMR graph based on node span matching. \heng{how do you handle ambiguity?}
Finally, we encode the KG enriched AMR graph using graph attention networks (GAT) that is able to incorporate fine-grained edge features before conducting IE tasks. \heng{here it would be good to refer back to the examples}
%We evaluate our model on the existing benchmark GENIA-2011 dataset.
In addition to the existing GENIA-2011 benchmark, we also aim to evaluate the effectiveness of our framework on topic-specific literature. Thus we have developed a new ontology and new paper corpus specifically labeled by medical professionals related to COVID-19.
Our model greatly outperforms the baseline by 5.8\%, and the most previous benchmark by 2.7\% in terms of absolute F1 score. \heng{need to update these numbers after COVID expt is done}


%%%%%%%%%%%%%%COMMENTS%%%%%%%%%%%%%%%


% The second challenge lies in the lack of sufficient context and background knowledge
% for understanding the entity mentions. We propose leveraging global topical coherence and linking relevant
% mentions simultaneously. Our hypothesis is that if multiple mentions co-occur in the same sentence, are
% linked through dependency paths, or play the same role in the same event, that they are probably
% semantically related; their reference entities are then connected via links to other documents.






% Moreover, a major bottleneck in understanding scientific literature lies in the enormous amount of unexplained abbreviations and terminologies. %For example, in order to understand terms like \emph{EGFR}, 
% We propose to apply our state-of-the-art Entity Linking techniques for general domain~\cite{Pan2015} and for biomedical literature~\cite{Zheng2014} to automatically link them to background KBs and ontologies, and then %. Then we propose to 
% capture such domain-specific knowledge using attention mechanisms. For example, \emph{EGFR} can be linked to \emph{Epidermal Growth Factor Receptor} or \emph{Estimated Glomerular Filtration Rate} in 300+ biomedical ontologies with confidence score $L$. We use $G$ to denote the distribution between its entity types in the KBs and paper dimensions, and $G$ can be optimized by the neural architecture. Thus for each word, we can get an additional paper dimension distribution vector $A=L\times G$ 
% %. We will concatenate the original semantic vector of each word with the paper dimension distribution vector 
% as input to Graph-LSTM.


%to solve two problems together, we propose a knowledge-enriched amr framework... give examples

%describe detailed method
%summarize results
%contributions...
% \heng{for both papers we need good examples to show why we need external knowledge, pick some examples where the concept is very hard to understand based on local sentence context only
% and for @Zixuan you also need to show some example where the distance between two entities, or between trigger and entity are very wide and thus you need amr parser to compress the context}
% \heng{add in stats/examples from Zixuan's slides}
% structure complex; need a good example to show amr graph can make the distance much shorter


% need external knowledge base; a lot of information is left unexplained; use ai institute words
% We propose to perform link prediction to enrich and refine the KGs by combining knowledge graph embedding and text embedding. 
% %One major remaining challenge %to meet COVID-19 question answering requirement 
% %is that our current system lacks of the ability to perform link prediction and reasoning. We propose a new entity representation that %combines KG structure and unstructured contextual text for link prediction. 
% %In addition, 
% We propose to leverage generative models to approximate the natural data distribution and capture the complicated structure of existing sub-graphs to further generate potential links.
% Most of the existing generative models aim to generate as diverse as possible graphs from the training set. On the other hand, our goal is to leverage the generative model to predict which edges are more likely to be generated, which means we hope to preserve the properties of original graph. Hence, we aim to design a generative model that could discover the graph structural pattern and does not need to include much diversity.



% combine text and knowledge representation
% Text structured representation. To incorporate the local context information, we will apply a bi-directional
% long short-term memory (LSTM)106 to encode sentences from tens of millions of papers. We will pre-train
% the state-of-the-art contextualized language model BERT encoder107 to learn joint entity and word
% embeddings. To further incorporate symbolic semantic information, we will run our Abstract Meaning
% Representation (AMR)108 semantic parser109 on sentences; AMR utilizes multi-layer linguistic analysis to
% represent the semantic graph structure of a sentence. We will also encode long-range relational information
% by applying Graph Convolutional Network (GCN)110 to encode the graph contextual information111 of AMR
% structures.



%\heng{two major challenges: 1. use amr parsing graph; 2. use external knowledge; test on biomedical, chemistry, covid, maybe also agriculture if we have data; 3. use new covid data}



% \textbf{Limitations of State-of-the-art.} Most previous studies apply supervised sequence labeling models~\cite{Lee2017,Segura-Bedmar2017,Ammar2017} or adopt semi-supervised learning% for bootstrapping
% ~\cite{Gupta2011,Tsai2013,Luan2017}. % and label propagation~\cite{Luan2017}. 
% The best end-to-end F-score for the {\em ScienceIE} shared task %concerned with extracting keyphrases and relations %from scientific papers 
% was only about 43\%~\cite{Ammar2017}. The features used are limited to lexical and syntactic analysis along with general word embeddings.
% %- this ignores rich semantic structure constraints in larger contexts and global background knowledge. 
% %In the following, we elaborate upon these major challenges and propose a novel solution.






% \begin{figure}[!htb]
% \vspace{-.15in}
% \includegraphics[width=\textwidth]{figs/attention1.pdf}
% \caption{AMR-based Attentive Graph-LSTM for Paper Dimension Extraction}
% \vspace{-.2in}
% \label{fig:dimensiondnn}
% \end{figure}
% %Bi-directional Long Short-Term Memory networks (Bi-LSTM)  meet this requirement by processing each sequence in both directions with two separate hidden layers, which are then fed into the same output layer. 




% \textbf{Challenges and Our Proposed Novel Approach:} Semantic structure-based patterns are crucial for paper dimension classification. For example, if we can determine the semantic role of \emph{Braf inhibition } as \emph{ARG1 (recipient)} of the predicate \emph{propose}, we can easily apply the domain-independent structure pattern <propose, ARG1, Technology> to label the dimension type of \emph{Braf inhibition } as \emph{Technology}. We propose to adopt the Abstract Meaning Representation (AMR)~\cite{banarescu13}. AMR is a semantic representation language, to convert the meaning of each input sentence into a rooted, directed, labeled, acyclic graph structure. AMR semantics includes PropBank frames, non-core semantic roles, coreference, entity typing and linking, modality, and negation. We have developed state-of-the-art automatic AMR semantic parsers~\cite{Pust2015,Wang2016}. Compared with dependency parsing and semantic role labeling, the nodes in AMR are concepts instead of words, and the edge types are much more fine-grained. A large, labeled AMR corpus has been developed  for both general domain and biomedical scientific literature domain.\footnote{Available at https://catalog.ldc.upenn.edu/LDC2017T10 and https://amr.isi.edu} Then we propose to adopt a Graph-LSTM framework to capture AMR graph structures. 
% %Unlike tree-LSTMs, graph-LSTM units may have multiple predecessors, and for each, there is a forget gate and a typed weight to signify the connection between the predecessor and the current unit. The weights of each connection type can be simultaneously optimized with the other parameters.
